Parallel Algorithms for Median Consensus Clustering in Complex Networks

We develop an algorithm that finds the consensus of many different clustering solutions of a graph. We formulate the problem as a median set partitioning problem and propose a greedy optimization technique. Unlike other approaches that find median set partitions, our algorithm takes graph structure into account and finds a comparable quality solution much faster than the other approaches. For graphs with known communities, our consensus partition captures the actual community structure more accurately than alternative approaches. To make it applicable to large graphs, we remove sequential dependencies from our algorithm and design a parallel algorithm. Our parallel algorithm achieves 35x speedup when utilizing 64 processing cores for large real-world graphs from single-cell experiments.

==> introduction.tex <==
\section{Introduction}
Finding clusters on a graph is of great importance in many applications, but defining clusters is challenging. 
Clusters are typically defined by processes, and different processes can find different clusters on the same graph. 
The stochastic nature of these processes means that the same process can find different clusters on the same graph. 
This leads to unreliable cluster detection~\cite{fortunato2010community}. 
In dynamic graphs where vertices and edges change over time, clusters detected at one time step become less reliable over time. 
Consensus clustering is seen as a way to find more reliable clusters\cite{lancichinetti2012consensus}.


The reliability of clusters is very important for many applications.
For example, Yadav et al. studied the resiliency of a practical infrastructure network under disruption over time period~\cite{yadav2020resilience}.
The US National Academy of Sciences defines resilience as the ability to plan and absorb such disruptive events~\cite{national2012disaster}.
Dong et al.~\cite{dong2018resilience} and Ramirez-Marquez et al.~\cite{ramirez2018quantifying}  emphasized the importance of clusters in quantifying network resilience.
Guerrero et al\cite{guerrero2018community} and Chen et al\cite{chen2015community} discussed the importance of finding clusters on electrical power grid graph for proper handling of disruptive events.
Hussain et al. argued that more resilient clusters can be found by modeling the problem as a consensus clustering problem~\cite{hussain2022disruption}.



Consensus clustering is a well-studied problem for data analytics.
Many different approaches has been studied to find consensus of different clustering of non-relational data ~\cite{vega2011survey}.
Most of these approaches are applicable for graphs if the edges are ignored.
However, as we have explored in this work, taking the graph structure into account can improve the performance of a consensus clustering algorithm in terms of both quality and computational resource requirements.

Existing works that create consensus taking graph structure into account are very limited.
Lancichinetti and Fortunato considered builiding a consensus matrix and applying the original graph clustering algorithm repeatedly until the consensus matrix does not change any more~\cite{lancichinetti2012consensus}.
This approach becomes prohibitive for large graphs because building and maintaining the consensus matrix consider all possible pairs of vertices which requires impractical amount of memory and runtime.
To alleviate this problem, Tandon et al. proposed an improvement that considers a significant subset of the pairs of vertices instead of all possible pairs~\cite{tandon2019fast}.
However, we observed that both of these approaches fail to converge to a solution when the variability of input clustering come from different clustering process rather than a single clustering algorithm.

Some recent works have considered clustering of clustering in order to improve reliability of graph clustering solutions.
Peixoto considers a probabilistic generative model that characterizes the similarity of each of the clustering solution to each other~\cite{peixoto2021revealing}.
Kirkley and Newman presents the clustering of clustering problem based on minimum description length principle~\cite{kirkley2022representative}.
The primary objective of this line of works is to capture similarity and dissimilarity between different clustering solutions.
Instead of creating a new consensus solution, these works represent each of the similar groups by one of the clustering solutions.
However, as we show in this work, creating consensus of each of the similar group of clustering improves the overall quality of clustering for each group.

\textbf{Our contribution}.
In this work we study the consensus clustering problem for a graph as finding a clustering solution that reduces the total distance between the consensus solution and all input clustering solutions.
There are many ways to define this distance~\cite{meilǎ2005comparing}.
We take inspiration from Filkov and Skienna~\cite{filkov2004integrating} and consider rand distance as the direct objective to optimize.
By taking the graph structure into account we introduce a greedy optimization heuristic.
Unlike the the graph-agnostic solution introduces by Filkov and Skienna~\cite{filkov2004integrating}, our algorithm does not suffer from high memory requirement and does not have sequential dependencies. 
Getting rid of the sequential dependencies enabled us to easily design a parallel algorithm as well.
We empirically show that our algorithm produces superior quality solutions compared to most of the other methods of finding consensus clustering in graphs.


